Toward Accurate and Temporally Consistent Video Restoration from Raw Data

Denoising and demosaicking are two fundamental steps in reconstructing a clean full-color video from raw data, while performing video denoising and demosaicking jointly, namely VJDD, could lead to better video restoration performance than performing them separately. In addition to restoration accuracy, another key challenge to VJDD lies in the temporal consistency of consecutive frames. This issue exacerbates when perceptual regularization terms are introduced to enhance video perceptual quality. To address these challenges, we present a new VJDD framework by consistent and accurate latent space propagation, which leverages the estimation of previous frames as prior knowledge to ensure consistent recovery of the current frame. A data temporal consistency (DTC) loss and a relational perception consistency (RPC) loss are accordingly designed. Compared with the commonly used flow-based losses, the proposed losses can circumvent the error accumulation problem caused by inaccurate flow estimation and effectively handle intensity changes in videos, improving much the temporal consistency of output videos while preserving texture details. Extensive experiments demonstrate the leading VJDD performance of our method in term of restoration accuracy, perceptual quality and temporal consistency. Codes and dataset are available at \url{https://github.com/GuoShi28/VJDD}.

==> sec/3_method.tex <==
\section{Method}

\subsection{Overall Framework}
The objective of video joint denoising and demosiacking (VJDD) is to reconstruct a clean RGB video $\mathcal{X} = \{ x_t \}_{t=1}^{N}$ from the mosaicked noisy raw video $\mathcal{Y} = \{ y_t \}_{t=1}^{N}$. Following the noise model proposed in~\cite{brooks2019unprocessing,guo2021joint}, the noisy frame $y_t$ can be modeled as:
\begin{equation}
    y_t = M(x_t)+n(M(x_t),\sigma_s,\sigma_r),
\label{eq:degrademodel}
\end{equation}
where $n(x, \sigma_s, \sigma_r) \sim \mathcal{N}(0, \sigma_s x + \sigma_r^2)$ is a Gaussian noise model with shot noise scale $\sigma_s$ and read noise scale $\sigma_r$, and $M(\cdot)$ denotes the mosaic downsampling operator. Compared to the JDD for a single image or burst images, VJDD also needs to keep the temporal consistency of video frames. To address this challenge, we propose a consistent latent space propagation framework with temporal regularizations for VJDD, as illustrated in \cref{fig:Overall} (a). 

Firstly, we extract shallow features $\{ I_t \}_{t=1}^{N}$ from the noisy frames $\{ y_t \}_{t=1}^{N}$ and their corresponding noise maps $\{ m_t \}_{t=1}^{N}$, which are formed by the standard deviations of signal-dependent Gaussian noise at each pixel. The extracted features are propagated by using our consistent latent space propagation strategy. Specifically, the features are aligned by the proposed global-to-local alignment module (GLAM), and then aggregated and fed into the reconstruction module (RCM), resulting in the reconstructed features $H_{t}$. The clean full color frames $\hat{x}_t$ are obtained by applying a $3\times 3$ convolution layer on $H_{t}$. The detailed structures of GLAM are shown in \cref{fig:Overall} (b), where we perform alignment in a global-to-local manner to increase the receptive filed of the alignment module, and the structure of RCM is shown in \cref{fig:Overall} (c), where we employ a 5-scale UNet with skip connections. The channel attention module (CAM) and spatial attention module (SAM) are used to enhance the feature extraction capability of the RCM, whose implementation details can be found in \cite{guo2021joint}. To ensure the temporal consistency, we introduce two loss functions, \ie, the data temporal consistency loss and the relational perceptual consistency loss, to promote the temporal coherence in the reconstructed video frames.

\subsection{Consistent Latent Space Propagation}
Propagation plays a crucial role in leveraging the information within a video sequence for restoration tasks. There are three types of commonly used methods: sliding-window propagation~\cite{isobe2020video,wang2019edvr,guo2021joint,guo2022differentiable}, recurrent propagation~\cite{sajjadi2018frame,isobe2020video2}, bidirectional recurrent propagation~\cite{chan2020basicvsr,huang2015bidirectional,huang2017video,chan2022basicvsr++}. Sliding-window propagation restricts the accessible information for reconstructing the $t$-th frame within a local neighborhood $(t-\lfloor n/2 \rfloor:t+ \lfloor n/2 \rfloor)$, where $n$ denotes the number of frames. Such an approach effectively utilizes the information of local frames but omits distant frames, and the reconstruction of frame $t$ is independent of that of frame $t-1$, which is prone to temporal inconsistency. Recurrent propagation sequentially aggregate information, and the reconstruction of frame $t$ depends on the reconstructed frame $t-1$, hence promoting temporal consistency. Nonetheless, this approach only exploits the information from previous frames and overlooks subsequent frames. Bidirectional recurrent propagation leverages information from both forward and backward frames; however, this strategy requires to store the hidden state of all frames, resulting in high memory usage for video processing. 

To efficiently utilize the redundant information among video frames and maintain temporal consistency, we present a consistent latent space propagation scheme, as shown in \cref{fig:Overall} (a). We employ the features of neighboring frames $I_{t-\lfloor n/2 \rfloor:t+ \lfloor n/2 \rfloor}$, referred to as the buffer frames, and recurrently employ the reconstruction feature of previous frame, denoted by $H_{t-1}$, to reconstruct the desired frame $x_t$. The features of input frames are first aligned with the feature of reference frame $I_t$ by using the GLAM module, and then concatenated as the input to the RCM module. By incorporating the reconstruction results of previous frames as prior information, we can enhance the inter-frame consistency in the final output video.

The efficiency of our proposed propagation scheme lies in  two aspects. First, to restore the current frame $t$, we only need to store the features of buffer frames and the reconstruction feature of previous frame (\ie, $H_{t-1}$), resulting in a memory-efficient framework compared to bidirectional recurrent propagation~\cite{chan2020basicvsr,chan2022basicvsr++}. Second, when restoring the next frame $t+1$, the buffer frame features can be efficiently updated by removing the feature of frame $t-\lfloor n/2 \rfloor$ and adding the feature of frame $t+\lfloor n/2 \rfloor+1$. This allows us to reuse the features of $n-1$ frames without re-calculation. Different from the propagation method employed in RLSP~\cite{fuoli2019efficient}, our approach focuses on propagating the locally neighboring frames in latent space and reusing their features, resulting in much less computational cost. In addition, we design an alignment module to compensate for the offset between frames, which is crucial to enhance the video restoration performance  ~\cite{wang2019edvr,guo2022differentiable}.

\subsection{Global-to-Local Alignment Module}
Alignment is a crucial component for VJDD. While previous studies~\cite{chan2022basicvsr++,chan2021understanding} have demonstrated the effectiveness of deformable alignment in feature space~\cite{wang2019edvr,guo2021joint}, it encounters difficulties in dealing with large shift due to the limited receptive field~\cite{guo2022differentiable}. To address this issue, we design a GLAM module by first handling the global motion between features and then employing deformable convolution (DConv) to achieve pixel-wise alignment.

The structure of GLAM is illustrated in  \cref{fig:Overall} (b). By taking the reference feature $I_t$ and the target feature $I_{t+1}$ as inputs, GLAM aims to spatially align $I_{t+1}$ with $I_t$. To enhance the alignment performance, we adopt a pyramid alignment strategy with three scales. Firstly, we estimate the global motion at $\frac{1}{4}$ resolution to reduce the computational cost by solving the following equation:  
\begin{equation}
    \hat{f}_{g}^{\frac{1}{4}} = \operatorname*{argmin}_{f \in [-f_{max}, f_{max}]} \Vert \tau(I_{t+1}^{\frac{1}{4}}, f) - I_{t}^{\frac{1}{4}} \Vert,
\end{equation}
where $\tau(I, f)$ shifts image $I$ with the estimated global translation $f$, and $f_{max}$ is the maximum motion field. The estimated global motion is employed to align features at all scales by rescaling $\hat{f}_{g}^{\frac{1}{4}}$ to the feature resolution of other scales. Then, pixel alignment is performed using DConv. On each pyramidal scale $s$, suppose we have the globally aligned features $\hat{I}_{t}^s$ and $\hat{I}_{t+1}^s$. The offset is estimated as:
\begin{equation}
\hat{f}_{p}^s = g_1(\text{LReLU}([g_2([\hat{I}_{t}^s,\hat{I}_{t+1}^s]), \hat{f}_{p}^{(s-1) \uparrow2}])),
\end{equation}
where $g_1$ and $g_2$ are two convolutional layers, $[\cdot,\cdot]$ is the concatenation operator, and $(\cdot)^{\uparrow 2}$ is the upsampling operator with factor 2. The aligned feature ${I'}_{t+1}^s$ is obtained by:
\begin{equation}
    {I'}_{t+1}^s = g([\text{DConv}(\hat{I}_{t+1}^s, \hat{f}_{p}^s), {I'}_{t+1}^{(s-1) \uparrow2}]),
\end{equation}
where $g$ refers to general Conv+LReLU layer.

\subsection{Temporal Consistency Loss}
The flow-based temporal loss has been widely used in video processing to improve the temporal consistency ~\cite{lai2018learning,lei2019fully,lai2018learning,wang2020consistent,park2019preserving}. While those losses can address the temporal consistency issue of low-frequency contents in tasks like video colorization and video style transfer, they are not well-suited for preserving the temporal consistency of high-frequency textures and structures in video restoration tasks. In addition, flow-based temporal losses often lead to the over-smoothing problem~\cite{dai2022video} due to the flow estimation errors. To solve these limitations, we design two new temporal losses for the VJDD task.

% \subsubsection{Data Temporal Consistency Loss}
\textbf{Data Temporal Consistency (DTC) Loss.}
The goal of DTC loss is to utilize the ground-truth optical flow to more precisely model the temporal consistency. During the training process, for a clean frame $x$, we randomly generate a sequence of optical flow $\{ f_{t\rightarrow t+1} \}_{t=1}^{N}$ from it. Then we synthesize a noisy raw video with the generated ground-truth optical flow by using $y_{t} = \mathcal{D}(\tau(x, f_{0\rightarrow t+1}),\sigma_s,\sigma_c)$, where $\mathcal{D}$ represents the degradation process described in \cref{eq:degrademodel}, and $f_{0\rightarrow t+1} = \sum_{k=0}^{t} f_{k\rightarrow k+1}$. Then the DTC loss can be defined as follows:
\begin{align}
    \mathcal{L}_{DTC} = \sum_{t=1}^{N-1}
    \Vert \tau(F(y_t), f_{t\rightarrow t+1}) - F(y_{t+1})\Vert,
\end{align}
where $F$ refers to our VJDD method. To account for long-term temporal consistency, we further introduce the long-term DTC loss, denoted as $\mathcal{L}_{DTC-l}$, as follows:
\begin{align}
    \mathcal{L}_{DTC-l} = \sum_{t=1}^{N-n}
    \Vert \tau(F(y_t), f_{t\rightarrow t+n}) - F(y_{t+n})\Vert.
\end{align}
By using the synthesized video to compute the temporal loss, $\mathcal{L}_{DTC}$ mitigates the error accumulation problem  of optical flow based temporal losses.

% \subsubsection{Relational Perceptual Consistency Loss}
\textbf{Relational Perception Consistency (RPC) Loss.}
The DTC loss $\mathcal{L}_{DTC}$ is limited in capturing real motions because it utilizes simulated motions in training. We therefore further design a RPC loss, denoted by $\mathcal{L}_{RPC}$, which leverages real videos for training. The RPC loss aims to model the perceptual temporal relationship between the restoration results and the ground-truth video.  Like \cite{eilertsen2019single,dai2022video}, we directly apply the RPC loss on the unaligned frames. The $\mathcal{L}_{RPC}$ is defined as follows:
\begin{equation}
\small
    \mathcal{L}_{RPC} = \sum_{t=1}^{N-1}\Vert (\Phi(\hat{x}_t) - \Phi(\hat{x}_{t+1})) - (\Phi(x_t) - \Phi(x_{t+1}))\Vert,
\end{equation}
\noindent where $\hat{x}_t$ and $x_t$ represent the VJDD output and the ground-truth, respectively. The function $\Phi(\cdot)$ extracts perceptual features to promote consistency in structure and texture regions between frames. We adopt the pre-trained VGG perceptual network \cite{johnson2016perceptual} as $\Phi(\cdot)$. The term $(\Phi(x_t) - \Phi(x_{t+1}))$ captures the ground-truth perceptual relationship between clean frames, encompassing the unaligned intensity differences of the video. By comparing the perceptual relationship of ground-truth video and estimated video, the value of $\mathcal{L}_{RPC}$ can measure the presence of temporal flickering artifacts between frames.

% ----- experiment results : value ------
{
\renewcommand{\arraystretch}{1.2}
\begin{table*}[!tbp]
%\setlength{\abovecaptionskip}{0.0cm}
%\setlength{\belowcaptionskip}{0.0cm}
%\footnotesize
\small
\centering
%\smallskip
\caption{Quantitative comparison of different VJDD approaches on the REDS4 and 4KPix50 dataset. Following the experiment setting of \cite{mildenhall2018burst,xu2019learning}, ``Low" and ``High" noise levels are corresponding to $\sigma_s = 2.5\times 10^{-3}$, $\sigma_r = 10^{-2}$ and $\sigma_s = 6.4\times 10^{-3}$, $\sigma_r = 2\times 10^{-2}$, respectively. The best results are highlighted in bold.} %\vspace{0.2cm}
\label{synthREDS4}
\begin{tabular}{c | c | c | c c c c c c c}
%\toprule
\hline
%& & &\multicolumn{2}{c}{Restoration Accuracy} &\multicolumn{2}{c}{Perceptual Quality}  &\multicolumn{2}{c}{Temporal Consistency} \\ 
%\midrule
Noise &Dataset &Method &PSNR $\uparrow$ &SSIM $\uparrow$ &LPIPS $\downarrow$ &DISTS $\downarrow$ &WE ($10^{-2}$) $\downarrow$ &tOF $\downarrow$ &RWE ($10^{-2}$) $\downarrow$ \\
\hline
\multirow{10}{*}{Low} &\multirow{5}{*}{REDS4}
&EDVR-VJDD &34.02 &0.9105 &0.0964 &0.0670 &$1.73\times 10^{-2}$ &0.3718 &$1.42\times 10^{-2}$  \\
& &RviDeNet-VJDD &34.86 &0.9221 &0.0884 &0.0636 &$1.78\times 10^{-2}$ &0.3742 &$1.46\times 10^{-2}$  \\
& &GCP-Net &36.20 &0.9383 &0.0845 &0.0584 &$1.30\times 10^{-2}$ &0.2889 &$1.08\times 10^{-2}$  \\
& &2StageAlign &36.59 &\textbf{0.9448} &0.0791 &0.0553 &$1.29\times 10^{-2}$ &0.2727 &$1.07\times 10^{-2}$ \\
%\cmidrule{3-10}
\cline{3-10}
& &Ours &\textbf{36.78} &0.9445 &\textbf{0.0654} &\textbf{0.0317} &$\mathbf{1.21\times 10^{-2}}$ &\textbf{0.2477} &$\mathbf{1.02\times 10^{-2}}$  \\

\cline{2-10}

&\multirow{5}{*}{4KPix50}
& EDVR-VJDD &36.36 &0.9415 &0.1006 &0.0776 &$1.14\times 10^{-2}$ &0.4941 &$9.9\times 10^{-3}$  \\
& &RviDeNet-VJDD &36.52 &0.9392 &0.0990 &0.0736 &$1.20\times 10^{-2}$ &0.4626 &$1.03\times 10^{-2}$  \\
& &GCPNet &38.13 &0.9503 &0.0859 &0.0631 &$8.2\times 10^{-3}$ &0.4166 &$7.6\times 10^{-3}$  \\
& &2StageAlign &38.16 &0.9570 &0.0853 &0.0644 &$8.4\times 10^{-3}$ &0.4279 &$7.8\times 10^{-3}$  \\
\cline{3-10}
& &Ours &\textbf{38.66} &\textbf{0.9576} &\textbf{0.0739} &\textbf{0.0424} &$\mathbf{7.9\times 10^{-3}}$ &\textbf{0.4201} &$\mathbf{7.2\times 10^{-3}}$  \\

%\cline{1-10}
\hline
\multirow{10}{*}{High} &\multirow{5}{*}{REDS4}
&EDVR-VJDD &32.06 &0.8715 &0.1421 &0.0887 &$1.94\times 10^{-2}$ &0.5433 &$1.74\times 10^{-2}$  \\
& &RviDeNet-VJDD &32.62 &0.8850 &0.1376 &0.0890 &$2.02\times 10^{-2}$ &0.5681 &$1.81\times 10^{-2}$  \\
& &GCP-Net &34.08 &0.9124 &0.1297 &0.0817 &$1.36\times 10^{-2}$ &0.4442 &$1.28\times 10^{-2}$ \\
& &2StageAlign &34.43 &0.9178 &0.1257 &0.0757 &$1.39\times 10^{-2}$ &0.4476 &$1.30\times 10^{-2}$  \\
\cline{3-10}
& &Ours &\textbf{34.72} &\textbf{0.9181} &\textbf{0.0977} &\textbf{0.0474} &$\mathbf{1.23\times 10^{-2}}$ &\textbf{0.3692} &$\mathbf{1.17\times 10^{-2}}$  \\

\cline{2-10}

&\multirow{5}{*}{4KPix50}
&EDVR-VJDD &34.62 &0.9188 &0.1415 &0.1033 &$1.28\times 10^{-2}$ &0.6349 &$1.20\times 10^{-2}$  \\
& &RviDeNet-VJDD &34.67 &0.9147 &0.1451 &0.1082 &$1.38\times 10^{-2}$ &0.6203 &$1.28\times 10^{-2}$  \\
& &GCP-Net &36.13 &0.9411 &0.1132 &0.0815 &$8.8\times 10^{-3}$ &0.5594 &$9.0\times 10^{-3}$  \\
& &2StageAlign &36.27 &0.9424 &0.1114 &0.0792 &$8.9\times 10^{-3}$ &0.5600 &$8.8\times 10^{-3}$  \\
\cline{3-10}
& &Ours &\textbf{36.96} &\textbf{0.9430} &\textbf{0.1002} &\textbf{0.0569} &$\mathbf{8.0\times 10^{-3}}$ &\textbf{0.5399} &$\mathbf{8.2\times 10^{-3}}$  \\

\hline
%\toprule
\end{tabular} 
%\end{tabularx} 
%\vspace{-0.2cm}
\label{table:reds4}
\end{table*}
}
% ---------- END TABLE -----------

\subsection{Overall Training Loss}
Following previous JDD methods~\cite{guo2021joint,guo2022differentiable}, we first define a reconstruction loss $\mathcal{L}_{r}$ in both linear RGB domain and sRGB domain:
\begin{equation}
\small
    \mathcal{L}_{r} = \sum_{t=1}^N \sqrt{\Vert \hat{x}_t - x_t \Vert^2 + \epsilon^2} + \sqrt{\Vert \Gamma(\hat{x}_t) - \Gamma(x_t) \Vert^2 + \epsilon^2},
\end{equation}
where $\Gamma(\cdot)$ is a predefined ISP operator and we adopt the one in \cite{brooks2019unprocessing}. Additionally, to obtain visually more pleasing VJDD results, the perceptual loss \cite{johnson2016perceptual} is also used:
\begin{equation}
    \mathcal{L}_{p} = \sum_{t=1}^N \sqrt{\Vert \Phi(\Gamma(\hat{x}_t)) - \Phi(\Gamma(x_t)) \Vert^2 + \epsilon^2}.
\end{equation}
The overall loss function is:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{r} + \lambda\mathcal{L}_{p} + \alpha\mathcal{L}_{DTC} + \beta\mathcal{L}_{DTC-l} + \gamma\mathcal{L}_{RPC},
\end{equation}
where $\lambda$, $\alpha$, $\beta$ and $\gamma$ are  balance parameters, and we empirically set them as 0.002, 0.5, 0.2 and 0.001, respectively, in all our experiments.

% ------- All 4K images ------
\begin{figure}[!tbp]
%\setlength{\abovecaptionskip}{0.5cm}
%\setlength{\belowcaptionskip}{-0.cm}
\centering
%\vspace{0.6cm}
%\hspace{-0.6cm}
\includegraphics[width=0.4\textwidth]{all_4K.jpg}\vspace{0.2cm}

\begin{overpic}[width=0.35\textwidth]{pixel_flow_hist_paper.png}
    \put(-5.0,15){\footnotesize \rotatebox{90}{Frequency}}
    \put(48,-4){\footnotesize Shift}
\end{overpic}%\vspace{0.4cm}

\caption{Top: scenes of our collected 4KPix50 videos. Bottom: distribution of motions of the 4KPix50 dataset.}
\label{fig:all_4K}
%\vspace{-0.2cm}
\end{figure}
% ------ END -----


%%% -------- REDS4 results on high noise level: 01 --------
\begin{figure*}[!h]
%\setlength{\abovecaptionskip}{0.2cm}
%\setlength{\belowcaptionskip}{-0.cm}
\centering
% Patch 2
\begin{minipage}[b]{1.0\textwidth}
\centering
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_noise_rgb.jpg}
    {\small (a) Noise image}
    \end{minipage} %\hspace{0.1cm}
    %
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_noise_rgb_patch.jpg}
    {\small (b) Noise patch}
    \end{minipage} %\hspace{0.1cm}
    %
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_edvr_jdd_patch.jpg}
    {\small (c) EDVR-VJDD~\cite{wang2019edvr}}
    \end{minipage} 
    %
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_rvidenet_jdd_patch.jpg}
    {\small (d) RviDeNet-VJDD~\cite{yue2020supervised}}
    \end{minipage} %\vspace{0.10cm}
\end{minipage}%\hspace{0.1cm}
\vspace{0.15cm}

\begin{minipage}[b]{1.0\textwidth}
\centering
%\hspace{4.42cm}
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_ours_guided_patch.jpg}
    {\small (e) GCP-Net~\cite{guo2021joint}}
    \end{minipage} %\hspace{0.1cm}
    %
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_PBMNet_patch.jpg}
    {\small (f) 2StageAlign~\cite{guo2022differentiable}}
    \end{minipage} %\hspace{0.1cm}
    %
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_RNN10_VGG_Aug_patch.jpg}
    {\small (g) Ours}
    \end{minipage} %\hspace{0.1cm}
    %
    \begin{minipage}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{REDS4_1/00000032_gt_patch.jpg}
    {\small (h) GT}
    \end{minipage} 
\end{minipage}%\hspace{0.1cm}
%\vspace{0.15cm}
\caption{VJDD results by different methods on \emph{Clip020} of the REDS4 dataset.}%\vspace{-0.4cm}
\label{fig:Reds4}
\end{figure*}
% ----------- END FIGURE -----------
